Beyond Blanket Masking: Examining Granularity for Privacy Protection in Images Captured by Blind and Low Vision Users

As visual assistant systems powered by visual language models (VLMs) become more prevalent, concerns over user privacy have grown, particularly for blind and low vision users who may unknowingly capture personal private information in their images. Existing privacy protection methods rely on coarse-grained segmentation, which uniformly masks entire private objects, often at the cost of usability. In this work, we propose FiGPriv, a fine-grained privacy protection framework that selectively masks only high-risk private information while preserving low-risk information. Our approach integrates fine-grained segmentation with a data-driven risk scoring mechanism. We evaluate our framework using the BIV-Priv-Seg dataset and show that FiG-Priv preserves +26% of image content, enhancing the ability of VLMs to provide useful responses by 11% and identify the image content by 45%, while ensuring privacy protection. Project Page: https://artcs1.github.io/VLMPrivacy/

==> sections/data.tex <==



==> sections/risk_v1.tex <==

% The risk scores are calculated with PageRank (\cite{page1999pagerank}) based algorithms. Briefly speaking, the original PageRank algorithm is used to determine the importance of web pages when an individual surfs the internet. To explain the PageRank based algorithms used in this paper, let us discuss the inherent properties shared between both website networks and personal identity information (PII) networks. 

% First, both website and PII networks can be constructed as direct graphs. For website networks, the nodes are websites and a link $(u, v)$ indicates that we can go from web page $u$ to web page $v$. For PII networks, the nodes are identity attributes and a link $(p, q)$ represents that losing identity attribute $p$ may cause the disclosure of $q$. 

% Second, the nodes of both website and PII networks have different importance attached to them. A website having more inward edges means the website is more importance. Similarly, a PII attribute having more inward edges shows it is more risky to be disclosed. 

% Based on the above similarities between website and PII networks, we use two PageRank based algorithms to calculate the risk scores associated with private objects. 

% If we run the PageRank algorithm on the World Wide Web network, we can get the PageRank coefficient for each node. The PageRank coefficient of a node represents the probability of an internet surfer randomly clicking the website represented by the node. Likewise, if we run the PageRank algorithm on a UTCID Identity Ecosystem graph, the coefficient of a node represents the probability of a PII attribute being disclosed. 

% For the first algorithm (shown as Algorithm \ref{alg-1}), we construct a UTCID Identity Ecosystem graph $G_1$ with ITAP dataset, assign the edge weights based on the occurrence frequency of each edge among the total identity theft and fraud cases in ITAP dataset, and apply the PageRank algorithm on the graph with each node $u$ having an importance value $\frac{loss[u]}{\sum_{u \in G_1} loss[u]}$, where $loss[u]$ is total loss amount associated with the node $u$. We can call the importance values of nodes ``initial importance''. 

% For the second algorithm (shown as Algorithm \ref{alg-2}), we still need to construct a UTCID Identity Ecosystem graph $G_2$ with ITAP dataset. Different from $G_1$, the edge weights are assigned based on the total loss amount of each edges $(u,v)$ among the total identity theft and fraud cases in ITAP dataset. Then we apply the PageRank algorithm on $G_2$. The initial importance for each node $u$ of $G_2$ is the total loss amount associated with the identity attribute node among the total identity theft and fraud cases contained in $G_2$, which is $\frac{loss[u]}{\sum_{u \in G_2} loss[u]}$. 

% The initial importance of nodes will be normalized to make sure the summation of the initial importance of all nodes in a graph $G$ equals to 1. We leverage the $pagerank$ function in NetworkX package to build the two PageRank based algorithms of Algorithm \cite{{alg-1}} and \cite{alg-2}. The error tolerance of convergence is set to $1e-6*len(G.nodes)$ where $len(G.nodes)$ is the length of the node list. 


% % \begin{algorithm}
% % \caption{PageRank Based Algorithm - 1}
% % \begin{algorithmic}
% % \State $G_1 \gets ITAPData$
% % \State \text{for $node$ in range($len(G_1.nodes)$):}
% % \State \text{\hspace{0.7cm} $initialImportance[node] = \frac{1}{len(G.nodes)}$}
% % \State \text{for $edge$ in range($len(G_1.edges)$):}
% % \State \text{\hspace{0.7cm} $weight[edge] = frequency(ITAPData, edge)$}
% % \State \text{PageRank($G_1$, $initialImportance$, $weight$)}
% % \end{algorithmic}
% % \label{alg-1}
% % \end{algorithm}

% % \begin{algorithm}
% % \caption{PageRank Based Algorithm - 2}
% % \begin{algorithmic}
% % \State $G_2 \gets ITAPData$
% % \State \text{for $node$ in range($len(G_2.nodes)$):}
% % \State \text{\hspace{0.7cm} $initialImportance[node] = lossAmount(ITAPData, node)$}
% % \State \text{for $edge$ in range($len(G_1.edges)$):}
% % \State \text{\hspace{0.7cm} $weight[edge] = lossAmount(ITAPData, edge)$}
% % \State \text{PageRank($G_1$, $initialImportance$, $weight$)}
% % \end{algorithmic}
% % \label{alg-2}
% % \end{algorithm}

% % \begin{algorithm}
% % \caption{PageRank Algorithm}
% % \begin{algorithmic}
% % \State $V \gets G.nodes$ 
% % \State $E \gets G.edges$
% % \State \text{for $v$ in $V$:}
% % \State \text{\hspace{0.7cm} $PageRankCoefficient[v] = \frac{1}{len(G.nodes)}$}
% % \State \text{for $u$ in G.nodes }:
% % \State \text{$PageRankCoefficient[u]$ = $\sum_{(v, u)\in E} PageRankCoefficient[v]*\frac{1}{degree(v)}$}
% % \end{algorithmic}
% % \label{alg}
% % \end{algorithm}
